The isometry group of the bounded Urysohn space is simple

We show that the isometry group of the bounded Urysohn space is simple. This extends previous work by the authors.

==> datum.tex <==
\newcommand{\datum}{buch1.0-58-g59fcfde, Tue Apr 17 23:14:20 2012 +0200}

